Eilenberg-MacLane spectra as equivariant Thom spectra

We prove that the $G$-equivariant mod $p$ Eilenberg--MacLane spectrum arises as an equivariant Thom spectrum for any finite, $p$-power cyclic group $G$, generalizing a result of Behrens and the second author in the case of the group $C_2$. We also establish a construction of $\mathrm{H}\underline{\mathbb{Z}}_{(p)}$, and prove intermediate results that may be of independent interest. Highlights include constraints on the Hurewicz images of equivariant spectra that admit norms, and an analysis of the extent to which the non-equivariant $\mathrm{H}\mathbb{F}_p$ arises as the Thom spectrum of a more than double loop map.

==> NonEquivariant.tex <==
\section{The non-equivariant story}\label{sec:nonequiv}

Both authors are fond of the following result of Mahowald
\cite{mahowald}:

\begin{theorem}[Mahowald] \label{thm:MahE2}
The Thom spectrum of the unique non-trivial double loop map
\begin{equation} \label{eqn:Mah}
\Omega^2 S^3 \longrightarrow \mathrm{BO}
\end{equation}
is $\mathrm{H}\mathbb{F}_2$.
\end{theorem}
\begin{remark} This result and several
variants have enjoyed many subsequent proofs
in the literature. Examples include \cite{mahowald-thom,
cohen-may-taylor,priddy,temss,akhil-niko-justin}.
\end{remark}


In modern language, Mahowald's theorem states that the free $\mathbb{E}_2$-algebra with $2=0$ is $\mathrm{H}\mathbb{F}_2$
(cf. \cite{omar-toby, akhil-niko-justin}), and so proves the nilpotence of all
simple $2$-torsion classes in the stable homotopy groups of spheres
\cite{nishida}.

Less well-known is that Mahowald's map (\ref{eqn:Mah}) is in fact a triple loop map, as revealed by the following observation:

\begin{obs} \label{obs:TripleLoop}
Mahowald's map (\ref{eqn:Mah}) may be obtained by thrice looping the composite
$$\mathbb{H}P^{\infty} \simeq \mathrm{BSp}(1) \longrightarrow \mathrm{BSp}
\simeq \mathrm{B}^5\mathrm{O} \stackrel{\eta}{\longrightarrow} \mathrm{B}^4\mathrm{O}$$
\end{obs}

\begin{remark} This observation, combined with one of the main theorems of Klang in
\cite{klang}, allows a quick computation of the $\mathbb{E}_3$-center
(or $\mathbb{E}_3$ topological Hochschild cohomology) of
$\mathrm{H}\mathbb{F}_2$:
	\[
	\mathrm{map}_{\mathsf{Mod}^{\mathbb{E}_3}_{\mathrm{H}\mathbb{F}_2}}
	(\mathrm{H}\mathbb{F}_2, \mathrm{H}\mathbb{F}_2)
	\cong F(\mathbb{H}P^{\infty}_+, \mathrm{H}\mathbb{F}_2).
	\]
In fact, a Borel equivariant precursor to our main theorem at
the prime 2 appears as Lemma $3.1$ in \cite{klang}, where it is used in an essential manner to compute the factorization homology of Eilenberg--Maclane spectra.
\end{remark}

\begin{remark}
The authors first learned of Observation \ref{obs:TripleLoop} from Mike Hopkins.  We give a $C_2$-equivariant generalization in Section \ref{sec:prime2}.
\end{remark}

The remainder of the section will be about the case $p>2$, where there is the following theorem of Hopkins \cite[Lemma 3.3]{temss}:

\begin{theorem}[Hopkins] \label{thm:Hop}
Let 
	\[
	S^3 \stackrel{1-p}{\longrightarrow} \mathrm{B}^3\mathrm{GL}_1(S^0_{(p)})
	\]
denote the class $1-p \in \pi_0(S_{(p)})^{\times} = 
\pi_3(\mathrm{B}^3\mathrm{GL}_1(S_{(p)})).$  Then, applying $\Omega^2$, one obtains a map
	\[
	\Omega^2 S^3 \longrightarrow \mathrm{BGL}_1(S^0_{(p)})
	\]
with Thom spectrum equivalent to $\mathrm{H}\mathbb{F}_p$.
\end{theorem}

In light of the situation at $p=2$, it is natural to wonder if the map
$$1-p:S^3 \longrightarrow \mathrm{B}^3 \mathrm{GL}_1(S^0_{(p)})$$
may be delooped.  We record here the fact that it \textit{cannot}, which the authors could not locate in the literature.  At the prime $p=3$, the map is not even an $H$-space map for the standard $H$-space structure on $S^3=\mathrm{SU}(2)$.  Crucially, we will see in Section \ref{sec:exotic} that the map \emph{is} an $H$-space map for a certain exotic $H$-space structure on $S^3$.

\begin{theorem}\label{thm:non-eqvt}
Let $S^0_p$ denote the $p$-complete sphere spectrum, and suppose that $p>2$.  Then there is no triple loop map
$$X \longrightarrow \mathrm{BGL}_1(S^0_{p}),$$
for any triple loop space $X$, that makes $\mathrm{H}\mathbb{F}_p$ as a Thom spectrum.
\end{theorem}

\begin{proof}
To avoid a lengthy digression, we defer the proof to Appendix \ref{sec:appendix}.
\end{proof}

\begin{remark}
The above theorem also implies that there can be no triple loop map $X \longrightarrow \mathrm{BGL}_1(S^0_{(p)})$ making $\mathrm{H}\mathbb{F}_p$ as a Thom spectrum.
\end{remark}

